Hydrostatic mass profiles in X-COP galaxy clusters

We present the reconstruction of hydrostatic mass profiles in 13 X-ray luminous galaxy clusters that have been mapped in their X-ray and SZ signal out to $R_{200}$ for the XMM-Newton Cluster Outskirts Project (X-COP). Using profiles of the gas temperature, density and pressure that have been spatially resolved out to (median value) 0.9 $R_{500}$, 1.8 $R_{500}$, and 2.3 $R_{500}$, respectively, we are able to recover the hydrostatic gravitating mass profile with several methods and using different mass models. The hydrostatic masses are recovered with a relative (statistical) median error of 3% at $R_{500}$ and 6% at $R_{200}$. By using several different methods to solve the equation of the hydrostatic equilibrium, we evaluate some of the systematic uncertainties to be of the order of 5% at both $R_{500}$ and $R_{200}$. A Navarro-Frenk-White profile provides the best-fit in nine cases out of 13, with the remaining four cases that do not show a statistically significant tension with it. The distribution of the mass concentration follows the correlations with the total mass predicted from numerical simulations with a scatter of 0.18 dex, with an intrinsic scatter on the hydrostatic masses of 0.15 dex. We compare them with the estimates of the total gravitational mass obtained through X-ray scaling relations applied to $Y_X$, gas fraction and $Y_{SZ}$, and from weak lensing and galaxy dynamics techniques, and measure a substantial agreement with the results from scaling laws, from WL at both $R_{500}$ and $R_{200}$ (with differences below 15%), from cluster velocity dispersions, but a significant tension with the caustic masses that tend to underestimate the hydrostatic masses by 40% at $R_{200}$. We also compare these measurements with predictions from alternative models to the Cold Dark Matter, like the "Emergent Gravity" and MOND scenarios.

==> eg_prof.tex <==
\hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A1644_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A1795_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2029_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2142_eg.pdf}
} \hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2255_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2319_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A3158_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A3266_eg.pdf}
} \hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A644_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A85_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/HydraA_eg.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/RXC1825_eg.pdf}
} \hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/ZW1215_eg.pdf}
}


==> m_chi2.tex <==
 Name & $\chi^2_{\epsilon}$ (DOF) & $\chi^2_{T}$ (DOF) & $\chi^2_{P}$ (DOF) & $\chi^2_{\rm TOT}$ (DOF) \\
A85 & 66.9 (70) & 86.1 (13) & 10.2 (7) & 163.2 (90) \\
A644 & 43.5 (68) & 48.0 (12) & 85.1 (6) & 171.6 (86) \\
A1644 & 72.0 (65) & 53.5 (12) & 2.2 (8) & 127.7 (85) \\
A1795 & 45.7 (65) & 31.3 (13) & 8.2 (7) & 85.2 (85) \\
A2029 & 31.2 (65) & 120.3 (14) & 11.3 (7) & 162.8 (86) \\
A2142 & 77.5 (65) & 23.5 (12) & 2.0 (7) & 103.0 (84) \\
A2255 & 16.1 (58) & 3.3 (8) & 6.5 (8) & 25.9 (74) \\
A2319 & 69.5 (69) & 168.9 (19) & 5.0 (7) & 143.4 (95) \\
A3158 & 41.9 (68) & 20.4 (11) & 2.4 (7) & 64.7 (86) \\
A3266 & 90.3 (69) & 122.7 (13) & 23.8 (7) & 236.8 (89) \\
HydraA & 99.0 (67) & 2235.3 (12) &  -- (--) & 2334.3 (79) \\
RXC1825 & 51.7 (57) & 22.9 (11) & 5.0 (8) & 79.6 (76) \\
ZW1215 & 32.1 (61) & 9.4 (12) & 13.4 (7) & 54.9 (80) \\


==> m_mod_BUR.tex <==
 Name & \multicolumn{4}{c}{BUR} \\ \\
  & kpc & $c$ & $\sigma_{T, int}$ & $\ln E$ \\
A85 & $188^{+9}_{-11}$ & $4.87^{+0.21}_{-0.19}$ & $0.060^{+0.013}_{-0.009}$ & -7.3 \\
A644 & $172^{+6}_{-7}$ & $5.64^{+0.16}_{-0.15}$ & $0.001^{+0.000}_{-0.000}$ & -6.8 \\
A1644 & $294^{+17}_{-16}$ & $2.74^{+0.13}_{-0.11}$ & $0.001^{+0.000}_{-0.000}$ & -3.7 \\
A1795 & $146^{+7}_{-6}$ & $5.86^{+0.22}_{-0.22}$ & $0.047^{+0.012}_{-0.009}$ & -6.8 \\
A2029 & $186^{+9}_{-10}$ & $5.73^{+0.25}_{-0.21}$ & $0.064^{+0.010}_{-0.009}$ & -14.2 \\
A2142 & $237^{+11}_{-11}$ & $4.59^{+0.19}_{-0.16}$ & $0.060^{+0.014}_{-0.010}$ & -12.4 \\
A2255 & $409^{+28}_{-28}$ & $2.31^{+0.14}_{-0.12}$ & $0.002^{+0.002}_{-0.001}$ & -2.9 \\
A2319 & $229^{+11}_{-13}$ & $4.68^{+0.23}_{-0.18}$ & $0.042^{+0.013}_{-0.012}$ & -9.2 \\
A3158 & $217^{+12}_{-13}$ & $3.90^{+0.21}_{-0.17}$ & $0.026^{+0.013}_{-0.022}$ & -5.3 \\
A3266 & $313^{+30}_{-26}$ & $3.44^{+0.26}_{-0.21}$ & $0.074^{+0.015}_{-0.013}$ & -14.2 \\
HydraA & $96^{+15}_{-11}$ & $7.01^{+0.53}_{-0.57}$ & $0.097^{+0.019}_{-0.013}$ & 688.4 \\
RXC1825 & $220^{+10}_{-10}$ & $3.86^{+0.15}_{-0.14}$ & $0.001^{+0.000}_{-0.000}$ & -4.5 \\
ZW1215 & $303^{+20}_{-19}$ & $3.30^{+0.15}_{-0.14}$ & $0.002^{+0.002}_{-0.001}$ & -4.7 \\


==> m_mod_EIN.tex <==
 Name & \multicolumn{4}{c}{EIN} \\ \\
  & kpc & $c$ & $\sigma_{T, int}$ & $\ln E$ \\
A85 & $636^{+40}_{-73}$ & $1.49^{+0.18}_{-0.08}$ & $0.026^{+0.021}_{-0.008}$ & 4.6 \\
A644 & $325^{+60}_{-53}$ & $2.99^{+0.52}_{-0.42}$ & $0.062^{+0.017}_{-0.012}$ & -12.7 \\
A1644 & $1119^{+107}_{-207}$ & $0.66^{+0.15}_{-0.06}$ & $0.005^{+0.047}_{-0.003}$ & -3.1 \\
A1795 & $480^{+23}_{-21}$ & $1.92^{+0.08}_{-0.07}$ & $0.009^{+0.007}_{-0.006}$ & 3.5 \\
A2029 & $571^{+29}_{-38}$ & $1.95^{+0.13}_{-0.08}$ & $0.020^{+0.010}_{-0.008}$ & -3.4 \\
A2142 & $866^{+42}_{-39}$ & $1.27^{+0.05}_{-0.05}$ & $0.001^{+0.000}_{-0.000}$ & -3.1 \\
A2255 & $959^{+97}_{-124}$ & $0.88^{+0.14}_{-0.09}$ & $0.002^{+0.009}_{-0.001}$ & -6.5 \\
A2319 & $403^{+46}_{-47}$ & $2.64^{+0.34}_{-0.26}$ & $0.067^{+0.017}_{-0.013}$ & -15.9 \\
A3158 & $530^{+34}_{-52}$ & $1.57^{+0.16}_{-0.09}$ & $0.004^{+0.028}_{-0.003}$ & -0.2 \\
A3266 & $765^{+61}_{-91}$ & $1.34^{+0.18}_{-0.10}$ & $0.057^{+0.015}_{-0.013}$ & -9.1 \\
HydraA & $299^{+33}_{-29}$ & $2.45^{+0.21}_{-0.21}$ & $0.046^{+0.009}_{-0.006}$ & 696.3 \\
RXC1825 & $495^{+26}_{-66}$ & $1.71^{+0.25}_{-0.08}$ & $0.002^{+0.011}_{-0.001}$ & -1.9 \\
ZW1215 & $1341^{+145}_{-161}$ & $0.75^{+0.10}_{-0.07}$ & $0.004^{+0.008}_{-0.002}$ & 1.1 \\


==> m_mod_HER.tex <==
 Name & \multicolumn{4}{c}{HER} \\ \\
  & kpc & $c$ & $\sigma_{T, int}$ & $\ln E$ \\
A85 & $914^{+55}_{-109}$ & $1.92^{+0.26}_{-0.09}$ & $0.027^{+0.019}_{-0.010}$ & 5.8 \\
A644 & $478^{+73}_{-74}$ & $3.73^{+0.67}_{-0.45}$ & $0.090^{+0.027}_{-0.022}$ & -10.5 \\
A1644 & $2026^{+230}_{-188}$ & $0.72^{+0.07}_{-0.06}$ & $0.001^{+0.001}_{-0.000}$ & -2.4 \\
A1795 & $721^{+31}_{-37}$ & $2.37^{+0.12}_{-0.09}$ & $0.017^{+0.016}_{-0.007}$ & 5.2 \\
A2029 & $925^{+69}_{-42}$ & $2.27^{+0.10}_{-0.13}$ & $0.028^{+0.008}_{-0.007}$ & -5.8 \\
A2142 & $1262^{+46}_{-49}$ & $1.63^{+0.06}_{-0.05}$ & $0.006^{+0.011}_{-0.004}$ & -2.7 \\
A2255 & $2235^{+203}_{-289}$ & $0.73^{+0.11}_{-0.05}$ & $0.001^{+0.001}_{-0.000}$ & -6.2 \\
A2319 & $674^{+55}_{-77}$ & $2.99^{+0.41}_{-0.22}$ & $0.068^{+0.014}_{-0.010}$ & -12.5 \\
A3158 & $1203^{+137}_{-80}$ & $1.36^{+0.09}_{-0.12}$ & $0.001^{+0.001}_{-0.000}$ & -0.4 \\
A3266 & $1952^{+285}_{-189}$ & $1.03^{+0.10}_{-0.12}$ & $0.036^{+0.008}_{-0.008}$ & -8.7 \\
HydraA & $473^{+64}_{-43}$ & $2.86^{+0.24}_{-0.26}$ & $0.055^{+0.010}_{-0.007}$ & 694.9 \\
RXC1825 & $913^{+49}_{-69}$ & $1.76^{+0.14}_{-0.09}$ & $0.002^{+0.007}_{-0.001}$ & 0.1 \\
ZW1215 & $1325^{+86}_{-113}$ & $1.38^{+0.12}_{-0.07}$ & $0.004^{+0.020}_{-0.002}$ & 1.4 \\


==> m_mod_ISO.tex <==
 Name & \multicolumn{4}{c}{ISO} \\ \\
  & kpc & $c$ & $\sigma_{T, int}$ & $\ln E$ \\
A85 & $190^{+9}_{-9}$ & $7.71^{+0.29}_{-0.28}$ & $0.057^{+0.011}_{-0.008}$ & -9.5 \\
A644 & $168^{+9}_{-12}$ & $9.03^{+0.59}_{-0.32}$ & $0.029^{+0.028}_{-0.027}$ & -6.2 \\
A1644 & $298^{+19}_{-13}$ & $4.50^{+0.16}_{-0.19}$ & $0.001^{+0.000}_{-0.000}$ & -4.0 \\
A1795 & $144^{+8}_{-6}$ & $9.45^{+0.32}_{-0.39}$ & $0.055^{+0.012}_{-0.008}$ & -8.5 \\
A2029 & $195^{+13}_{-10}$ & $8.81^{+0.37}_{-0.39}$ & $0.078^{+0.015}_{-0.012}$ & -15.4 \\
A2142 & $240^{+13}_{-11}$ & $7.35^{+0.27}_{-0.26}$ & $0.060^{+0.011}_{-0.008}$ & -13.5 \\
A2255 & $444^{+42}_{-41}$ & $3.62^{+0.28}_{-0.22}$ & $0.001^{+0.001}_{-0.000}$ & -2.3 \\
A2319 & $241^{+14}_{-9}$ & $7.22^{+0.23}_{-0.32}$ & $0.041^{+0.018}_{-0.009}$ & -8.4 \\
A3158 & $223^{+15}_{-13}$ & $6.19^{+0.33}_{-0.29}$ & $0.030^{+0.009}_{-0.011}$ & -5.8 \\
A3266 & $312^{+30}_{-21}$ & $5.61^{+0.31}_{-0.30}$ & $0.076^{+0.015}_{-0.013}$ & -13.4 \\
HydraA & $221^{+63}_{-31}$ & $6.22^{+0.45}_{-0.42}$ & $0.324^{+0.029}_{-0.028}$ & 687.0 \\
RXC1825 & $233^{+10}_{-9}$ & $5.98^{+0.19}_{-0.18}$ & $0.001^{+0.001}_{-0.000}$ & -6.6 \\
ZW1215 & $313^{+18}_{-16}$ & $5.25^{+0.19}_{-0.17}$ & $0.001^{+0.000}_{-0.000}$ & -6.0 \\


==> m_mod_NFW.tex <==
 Name & \multicolumn{4}{c}{NFW} \\ \\
  & kpc & $c$ & $\sigma_{T, int}$ & $\ln E$ \\
A85 & $1921^{+30}_{-24}$ & $3.31^{+0.13}_{-0.13}$ & $0.019^{+0.012}_{-0.005}$ & 7.5 \\
A644 & $1847^{+61}_{-58}$ & $5.58^{+0.65}_{-0.51}$ & $0.063^{+0.017}_{-0.016}$ & -9.7 \\
A1644 & $1778^{+55}_{-48}$ & $1.46^{+0.14}_{-0.14}$ & $0.001^{+0.000}_{-0.000}$ & -2.5 \\
A1795 & $1755^{+22}_{-21}$ & $4.55^{+0.16}_{-0.14}$ & $0.009^{+0.012}_{-0.007}$ & 9.0 \\
A2029 & $2173^{+35}_{-33}$ & $4.26^{+0.19}_{-0.17}$ & $0.023^{+0.006}_{-0.005}$ & -2.5 \\
A2142 & $2224^{+29}_{-25}$ & $3.14^{+0.10}_{-0.10}$ & $0.001^{+0.000}_{-0.000}$ & -0.6 \\
A2255 & $2033^{+88}_{-74}$ & $1.37^{+0.24}_{-0.23}$ & $0.002^{+0.006}_{-0.001}$ & -4.2 \\
A2319 & $2040^{+34}_{-30}$ & $4.86^{+0.51}_{-0.37}$ & $0.055^{+0.009}_{-0.008}$ & -12.4 \\
A3158 & $1766^{+34}_{-37}$ & $2.88^{+0.26}_{-0.17}$ & $0.002^{+0.015}_{-0.001}$ & 1.2 \\
A3266 & $2325^{+74}_{-75}$ & $2.04^{+0.25}_{-0.20}$ & $0.036^{+0.008}_{-0.009}$ & -7.1 \\
HydraA & $1360^{+58}_{-55}$ & $5.51^{+0.67}_{-0.61}$ & $0.079^{+0.020}_{-0.016}$ & 698.1 \\
RXC1825 & $1719^{+24}_{-25}$ & $3.35^{+0.20}_{-0.19}$ & $0.001^{+0.001}_{-0.000}$ & 1.7 \\
ZW1215 & $2200^{+74}_{-64}$ & $2.11^{+0.22}_{-0.18}$ & $0.003^{+0.006}_{-0.002}$ & 5.4 \\


==> m_over.tex <==
\setlength{\tabcolsep}{3pt} % default value: 6pt
\begin{tabular}{c c c ccc cccc} \hline \hline
Name & $z$ & $c_{200}$ & 0.5 Mpc & 1 Mpc & 1.5 Mpc & $R_{500}$ & $M_{500}$ & $R_{200}$ & $M_{200}$ \\
 & & & $10^{14} M_{\odot}$ & $10^{14} M_{\odot}$ & $10^{14} M_{\odot}$ & Mpc & $10^{14} M_{\odot}$ & Mpc & $10^{14} M_{\odot}$ \\
A85 & 0.0555 & $3.31^{+0.13}_{-0.13}$ & $1.94 \pm 0.02$ & $4.53 \pm 0.08$ & $6.81 \pm 0.18$ & $1.235 \pm 0.013$ & $5.65 \pm 0.18$ & $1.921 \pm 0.027$ & $8.50 \pm 0.36$ \\ 
A644 & 0.0704 & $5.58^{+0.65}_{-0.51}$ & $2.36 \pm 0.09$ & $4.74 \pm 0.26$ & $6.59 \pm 0.45$ & $1.230 \pm 0.035$ & $5.66 \pm 0.48$ & $1.847 \pm 0.059$ & $7.67 \pm 0.73$ \\ 
A1644 & 0.0473 & $1.46^{+0.14}_{-0.14}$ & $1.15 \pm 0.02$ & $3.24 \pm 0.10$ & $5.47 \pm 0.26$ & $1.054 \pm 0.020$ & $3.48 \pm 0.20$ & $1.778 \pm 0.051$ & $6.69 \pm 0.58$ \\ 
A1795 & 0.0622 & $4.55^{+0.16}_{-0.14}$ & $1.95 \pm 0.02$ & $4.06 \pm 0.08$ & $5.77 \pm 0.15$ & $1.153 \pm 0.012$ & $4.63 \pm 0.14$ & $1.755 \pm 0.021$ & $6.53 \pm 0.23$ \\ 
A2029 & 0.0773 & $4.26^{+0.19}_{-0.17}$ & $2.78 \pm 0.03$ & $6.25 \pm 0.13$ & $9.24 \pm 0.26$ & $1.423 \pm 0.019$ & $8.82 \pm 0.35$ & $2.173 \pm 0.034$ & $12.57 \pm 0.59$ \\ 
A2142 & 0.0909 & $3.14^{+0.10}_{-0.10}$ & $2.48 \pm 0.02$ & $6.08 \pm 0.09$ & $9.44 \pm 0.19$ & $1.424 \pm 0.014$ & $8.95 \pm 0.26$ & $2.224 \pm 0.027$ & $13.64 \pm 0.50$ \\ 
A2255 & 0.0809 & $1.37^{+0.24}_{-0.23}$ & $1.39 \pm 0.06$ & $4.08 \pm 0.11$ & $7.10 \pm 0.36$ & $1.196 \pm 0.026$ & $5.26 \pm 0.34$ & $2.033 \pm 0.081$ & $10.33 \pm 1.23$ \\ 
A2319 & 0.0557 & $4.86^{+0.51}_{-0.37}$ & $2.61 \pm 0.08$ & $5.58 \pm 0.12$ & $8.01 \pm 0.25$ & $1.346 \pm 0.017$ & $7.31 \pm 0.28$ & $2.040 \pm 0.035$ & $10.18 \pm 0.52$ \\ 
A3158 & 0.0597 & $2.88^{+0.26}_{-0.17}$ & $1.59 \pm 0.02$ & $3.76 \pm 0.09$ & $5.70 \pm 0.21$ & $1.123 \pm 0.016$ & $4.26 \pm 0.18$ & $1.766 \pm 0.035$ & $6.63 \pm 0.39$ \\ 
A3266 & 0.0589 & $2.04^{+0.25}_{-0.20}$ & $2.02 \pm 0.05$ & $5.57 \pm 0.15$ & $9.32 \pm 0.39$ & $1.430 \pm 0.031$ & $8.80 \pm 0.57$ & $2.325 \pm 0.074$ & $15.12 \pm 1.44$ \\ 
HydraA & 0.0538 & $5.51^{+0.67}_{-0.61}$ & $1.28 \pm 0.07$ & $2.40 \pm 0.20$ & $3.22 \pm 0.32$ & $0.904 \pm 0.032$ & $2.21 \pm 0.23$ & $1.360 \pm 0.056$ & $3.01 \pm 0.37$ \\ 
RXC1825 & 0.0650 & $3.35^{+0.20}_{-0.19}$ & $1.64 \pm 0.02$ & $3.69 \pm 0.07$ & $5.46 \pm 0.15$ & $1.105 \pm 0.012$ & $4.08 \pm 0.13$ & $1.719 \pm 0.024$ & $6.15 \pm 0.26$ \\ 
ZW1215 & 0.0766 & $2.11^{+0.22}_{-0.18}$ & $1.93 \pm 0.03$ & $5.22 \pm 0.15$ & $8.61 \pm 0.39$ & $1.358 \pm 0.031$ & $7.66 \pm 0.52$ & $2.200 \pm 0.069$ & $13.03 \pm 1.23$ \\ 
\hline \end{tabular}


==> m_syst.tex <==
\setlength{\tabcolsep}{2pt} % default value: 6pt
\begin{tabular}{c c c c c c} \hline \hline
$M_i$ & \multicolumn{5}{c}{$B$ (inter-quartile range) \%} \\
  &  0.5 Mpc & 1 Mpc & 1.5 Mpc & $R_{500}$ & $R_{200}$ \\ \\
Forw & $+0.6 \, (-1.1/+3.3)$  & $-2.0 \, (-5.9/+1.4)$  & $-4.6 \, (-7.9/+1.3)$  & $-4.7 \, (-10.9/-0.5)$  & $+1.2 \, (-5.4/+8.1)$  \\
Forw (no SZ) & $-1.5 \, (-3.4/+4.1)$  & $-1.9 \, (-8.0/+0.6)$  & $-1.3 \, (-5.4/+4.5)$  & $-4.2 \, (-9.0/+1.8)$  & $+1.3 \, (-11.9/+8.0)$  \\
 \\
EIN & $-0.3 \, (-1.7/+1.3)$  & $-1.7 \, (-6.5/-0.2)$  & $-1.0 \, (-9.7/+1.5)$  & $-0.8 \, (-7.6/+1.0)$  & $-0.8 \, (-10.3/+4.3)$  \\
ISO & $+14.1 \, (+11.8/+21.0)$  & $-3.0 \, (-3.5/+5.4)$  & $-13.3 \, (-19.0/-9.7)$  & $-8.2 \, (-13.0/-5.3)$  & $-23.5 \, (-28.7/-16.5)$  \\
BUR & $+11.4 \, (+10.4/+15.1)$  & $-3.1 \, (-5.8/+4.0)$  & $-13.7 \, (-19.2/-8.3)$  & $-8.3 \, (-12.9/-5.2)$  & $-20.8 \, (-24.2/-17.9)$  \\
HER & $+1.6 \, (+0.9/+2.1)$  & $-0.7 \, (-5.6/+0.2)$  & $-5.5 \, (-11.4/-2.4)$  & $-3.7 \, (-5.3/-1.9)$  & $-9.3 \, (-13.5/-6.8)$  \\
\hline \end{tabular}


==> mprof.tex <==
\hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A1644_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A1795_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2029_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2142_mprof.pdf}
} \hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2255_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A2319_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A3158_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A3266_mprof.pdf}
} \hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A644_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/A85_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/HydraA_mprof.pdf}
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/RXC1825_mprof.pdf}
} \hbox{
\includegraphics[width=0.245\textwidth, keepaspectratio]{figs/ZW1215_mprof.pdf}
}

